Towards Understanding and Evaluating Structural Node Embeddings

While most network embedding techniques model the proximity between nodes in a network, recently there has been significant interest in structural embeddings that are based on node equivalences, a notion rooted in sociology: equivalences or positions are collections of nodes that have similar roles--i.e., similar functions, ties or interactions with nodes in other positions--irrespective of their distance or reachability in the network. Unlike the proximity-based methods that are rigorously evaluated in the literature, the evaluation of structural embeddings is less mature. It relies on small synthetic or real networks with labels that are not perfectly defined, and its connection to sociological equivalences has hitherto been vague and tenuous. With new node embedding methods being developed at a breakneck pace, proper evaluation and systematic characterization of existing approaches will be essential to progress. To fill in this gap, we set out to understand what types of equivalences structural embeddings capture. We are the first to contribute rigorous intrinsic and extrinsic evaluation methodology for structural embeddings, along with carefully-designed, diverse datasets of varying sizes. We observe a number of different evaluation variables that can lead to different results (e.g., choice of similarity measure, classifier, label definitions). We find that degree distributions within nodes' local neighborhoods can lead to simple yet effective baselines in their own right and guide the future development of structural embedding. We hope that our findings can influence the design of further node embedding methods and also pave the way for more comprehensive and fair evaluation of structural embedding methods.

==> 020related.tex <==

\noindent \textbf{Understanding Latent Representations.} 
Unsupervised latent feature representations or embeddings have been applied to a wide variety of objects\footnote{\url{https://github.com/MaxwellRebo/awesome-2vec}}, having been shown to yield powerful performance on downstream tasks.  However, because these are latent features, it is difficult to interpret them, thus it is unclear why certain methods do well or how to evaluate them.  
The NLP community has taken this challenge very seriously.  Prominent works have as their  objective the standardization of evaluation of word embeddings~\cite{schnabel2015evaluation}.  Other works have pointed out additional evaluation methods and challenges to the point where a multi-year workshop has arisen dedicated to the evaluation of word embeddings\footnote{\url{https://repeval2019.github.io/}}, and the field of word embedding evaluation now warrants a survey~\cite{bakarov2018survey}. 


Node embedding, being a comparatively newer area of study, is only now starting to see similar growth.  A few recent works~\cite{goyal2019benchmarks,gurukar2019network} benchmark the performance of popular node embedding algorithms on a variety of tasks and datasets.  This can be seen as a form of \emph{extrinsic} evaluation of the embeddings in the context of downstream tasks. Large-scale \emph{intrinsic} evaluation of node embedding is not as common, but another work has sought to understand various proximity-based node embedding methods by seeing what common centralities they are capable of predicting~\cite{dalmia2018towards}.  All of the above works, however, focus exclusively on embedding methods that preserve similarity in the latent feature space between nodes that are in close \emph{proximity} in the network. Interest in structural embeddings, has been growing, however, and a recent survey distinguishes them from proximity-preserving embeddings~\cite{rossi2019community}.   A standardized analysis of structural embedding methods is essential to ensure that the problem area indeed continues to see forward progress.   

\vspace{0.2cm}
\noindent \textbf{Node Embeddings.}
\label{sec:related-emb}
Node embedding is a function mapping nodes $V$ in a network $G$ to $d$-dimensional feature vectors $\mathbf{x}\in\mathbb{R}^d$ such that ``similar'' vertices have similar feature vectors, {based on some similarity measure}.   
Among the many existing techniques, our study focuses on methods that assume two nodes are similar if they have similar structural roles (defined in Section~\ref{sec:equivalences}) \textit{regardless} of their proximity in the network, and `hybrid' approaches 
(i.e., that capture both proximity and structural similarity to some extent).  We refer the reader to ~\cite{rossi2019community} for  more information on this distinction. 

$\bullet$ \textbf{Proximity-preservinng methods.} In our analysis, we consider two embedding methods that are primarily proximity-based. 
\textbf{(1)~node2vec}~\cite{node2vec} uses the skip-gram architecture~\cite{word2vec} to learn an embedding for each node that preserves its similarity to other nodes in its context, sampled with biased random walks. 
\textbf{(2)~LINE}~\cite{line} optimizes an embedding objective that maximizes the probability of the first and second-order proximities in the network (direct edges between any two nodes and mutual neighbors that any two nodes share, resp.).  
Proximity-preserving node embeddings are the topic of numerous surveys~\cite{gemsurvey,rossi2019community}, and we refer the interested reader to those. 

$\bullet$ \textbf{Structural methods.} We also evaluate {eight} structural embedding methods: 
\textbf{(3)~struc2vec}~\cite{struc2vec} uses the same skip-gram architecture, but samples context with random walks performed over an auxiliary multilayer graph capturing structural similarity (mainly \textit{degree}) of nodes' neighborhoods at several hop distances.  
\textbf{(4)~GraphWave} \cite{graphwave} computes the heat kernel matrix for a graph and embeds each node by sampling the empirical characteristic function of the distribution of heat it sends to other nodes.
\textbf{(5)~xNetMF}~\cite{xnetmf} draws on the connection between the skip-gram architecture matrix factorization~\cite{levy2014neural} to find node embeddings that implicitly factorize a structural similarity matrix, 
defined by comparing the distribution of node degrees in $k$-hop neighborhoods. 
{Subsequently, \textbf{(6) SEGK}~\cite{segk} factorizes a structural similarity matrix using graph kernels to compare the nodes' $k$-hop neighborhoods.} 
\textbf{(7)~role2vec}~\cite{role2vec} applies the skip-gram model to a corpus sampled using \emph{attributed} random walks which record the structural type of each node. The method learns the same embedding for nodes of each structural type, which enhances space efficiency. 
{\textbf{(8)~RiWalk}~\cite{riwalk} also uses the skip-gram model, but learns an embedding for each node based on the structural types of nodes in its context.}  
\textbf{(9)~DRNE}~\cite{drne} contends that feature propagation is similar to the recursive definition of regular equivalence, and uses an LSTM to learn node embeddings by aggregating the features of their neighbors sorted sequentially by degree.  
\textbf{(10)~MultiLENS}~\cite{multilens}, similar to xNetMF, derives embeddings based on matrix factorization that captures the distribution of structural features in nodes' local neighborhoods. 
In our analysis, we study the connections between these methods and the equivalence theory in social science.


==> dfn.tex <==
\newcommand{\reminder}[1]{{\textsf{\color{red}[#1]}}}
\newcommand{\addmore}{\reminder{...}}
\newcommand{\tara}[1]{{\textsf{\color{pink}[TS: #1]}}}
\newcommand{\davide}[1]{{\textsf{\color{blue}[DM: #1]}}}
\newcommand{\dk}[1]{{\textsf{\color{orange}[DK: #1]}}}

\newcommand{\placeholder}{... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... \\}


\newcommand{\method}{{{\textsc{GLIMPSE}}}}
\newcommand{\methodOffline}{{\textsc{QuotE-Offline}}}
\newcommand{\methodOnline}{{\textsc{QuotE-Online}}}
\newcommand{\greedy}{{\textsc{Greedy}}}
\newcommand{\methodFreq}{{{\textsc{QuotE-Freq}}}}
\newcommand{\methodRWR}{{{\textsc{QuotE-RWR}}}}
\newcommand{\rdf}{{\textsc{RDF}}}
\newcommand{\tcm}{{\textsc{TCM}}}
\newcommand{\tcmUser}{{\textsc{TCM-User}}}
\newcommand{\tcmConstrained}{{\textsc{TCM-Constrained}}}
\newcommand{\tcmRWR}{{\textsc{TCM-RWR}}}
\newcommand{\queryPres}{\textsc{Query-Pres}}
\newcommand{\cache}{\textsc{Cache}}
\newcommand{\cacheEntities}{\textsc{Cache-E}}
\newcommand{\topK}{\textsc{Top-K}}
\newcommand{\random}{\textsc{Random}}
\newcommand{\focused}{\texttt{F}}
\newcommand{\dispersed}{\texttt{D}}


\newcommand{\newpar}[1]{\vspace{.1cm}\noindent \textbf{#1}.}
\newcommand{\smallComment}[1]{\Statex{\textcolor{gray}{\texttt{// {#1}}}}}
\newtheorem{observation}{Observation}
\newtheorem{problem}{Problem}
\newtheorem{algo}{Algorithm}
\newtheorem{example}{Example}
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}


\newcommand{\argmax}[1]{\underset{#1}{\operatorname{arg}\,\operatorname{max}}\;}
\newcommand{\realNumbers}{\mathbb{R}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\expectation}{\mathbb{E}}
\newcommand{\indicator}{\textbf{1}}

\newcommand{\KG}{\mathcal{G}}
\newcommand{\summary}{\mathcal{S}}
\newcommand{\optimalSummary}{\summary^*}
\newcommand{\V}{\mathcal{V}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\entities}{\mathcal{E}}
\newcommand{\relationships}{\mathcal{R}}
\newcommand{\triples}{\mathcal{T}}
\newcommand{\entity}{e}
\newcommand{\relationship}{r}
\newcommand{\triple}{x_{ijk}}
\newcommand{\tripleLong}{(\entity_i, \relationship_k, \entity_j)}
\newcommand{\query}{Q}
\newcommand{\queries}{\mathcal{Q}}
\newcommand{\trainingQueries}{\queries{}_{\textrm{train}}}
\newcommand{\testingQueries}{\queries{}_{\textrm{test}}}
\newcommand{\budget}{B}
\newcommand{\cardinalityConstraint}{k}
\newcommand{\cost}{C}
\newcommand{\utility}{U}
\newcommand{\mappingTable}{\mathcal{T}}
\newcommand{\curvature}{\kappa}

\newcommand{\laplacian}{\textbf{L}}
\newcommand{\adjmat}{\textbf{A}}
\newcommand{\outdegree}[1]{d_{#1}^{+}}
\newcommand{\indegree}[1]{d_{#1}^{-}}
\newcommand{\heat}{u}
\newcommand{\heatVector}{\textbf{h}}
\newcommand{\queryVector}{\textbf{q}}
\newcommand{\I}{\textbf{I}}
\newcommand{\D}{\textbf{D}}
\newcommand{\M}{\textbf{M}}
\newcommand{\X}{\textbf{X}}
\newcommand{\vecr}{\textbf{r}}
\newcommand{\vecq}{\textbf{q}}
\newcommand{\vecx}{\textbf{x}}
\newcommand{\vecy}{\textbf{y}}
\newcommand{\diffusionMatrix}{\textbf{H}}
\newcommand{\simMatrix}{\textbf{S}}
\newcommand{\utilityVector}{\textbf{u}}
\newcommand{\modularUpperBound}{M}

\newcommand{\MAG}{\texttt{MAG}}
\newcommand{\DBIS}{\texttt{DBIS}}
\newcommand{\movies}{\texttt{Movies}}
\newcommand{\YAGO}{\texttt{YAGO}}
\newcommand{\DBPedia}{\texttt{DBPedia}}
\newcommand{\Freebase}{\texttt{Freebase}}

\newcommand{\nodeType}{\phi}
\newcommand{\edgeType}{\psi}
\newcommand{\nodeUtil}{u_{{\scriptscriptstyle \entities}}}
\newcommand{\edgeUtil}{u_{{\scriptscriptstyle \triples}}}
\newcommand{\nodeCost}{\phi}
\newcommand{\edgeCost}{\psi}
\newcommand{\entityCost}{\phi}
\newcommand{\relationshipCost}{\psi}
\newcommand{\intCost}{C_{ID}}

\newcommand{\timeHorizon}{T}
\newcommand{\totalReward}{U}

\definecolor{mygreen}{RGB}{34,139,34}




